Adaptive and Dynamic Multi-Resolution Hashing for Pairwise Summations

In this paper, we propose Adam-Hash: an adaptive and dynamic multi-resolution hashing data-structure for fast pairwise summation estimation. Given a data-set $X \subset \mathbb{R}^d$, a binary function $f:\mathbb{R}^d\times \mathbb{R}^d\to \mathbb{R}$, and a point $y \in \mathbb{R}^d$, the Pairwise Summation Estimate $\mathrm{PSE}_X(y) := \frac{1}{|X|} \sum_{x \in X} f(x,y)$. For any given data-set $X$, we need to design a data-structure such that given any query point $y \in \mathbb{R}^d$, the data-structure approximately estimates $\mathrm{PSE}_X(y)$ in time that is sub-linear in $|X|$. Prior works on this problem have focused exclusively on the case where the data-set is static, and the queries are independent. In this paper, we design a hashing-based PSE data-structure which works for the more practical \textit{dynamic} setting in which insertions, deletions, and replacements of points are allowed. Moreover, our proposed Adam-Hash is also robust to adaptive PSE queries, where an adversary can choose query $q_j \in \mathbb{R}^d$ depending on the output from previous queries $q_1, q_2, \dots, q_{j-1}$.

==> checklist.tex <==
\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} 
  \item Did you describe the limitations of your work?
    \answerYes{} We discuss the theoretical guarantees for accuracy-efficiency trade-off in Section~\ref{sec:adaptive_and_dynamic_hbe}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} Please refer to Section~\ref{sec:time_adaptive_hbe}. We discuss the running time complexity, which relates to the energy consumption in practice.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
   \answerYes{} 
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} Please refer to the supplementary materials.
        \item Did you include complete proofs of all theoretical results?
    \answerYes{} Please refer to Section~\ref{sec:adaptive_and_dynamic_hbe} supplementary materials.
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
   \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}
\end{enumerate}


\end{enumerate}

==> missing_proofs.tex <==
\section{Proofs for \textsc{InsertX} and \textsc{DeleteX}}\label{sec:missing_proofs}
In this section we prove the time complexity of \textsc{InsertX} and \textsc{DeleteX} operations in our Adam-Hash data structure.
\subsection{Running time of \textsc{InsertX}}\label{sec:adaptive_multi_insert_time_app}
The goal of this section is to prove the time complexity of \textsc{InsertX} operation.

\begin{lemma}[Restatement of Lemma~\ref{lem:adaptive_multi_insert_time}]
Given an estimator $Z$ of complexity $C$ which is $V$-bounded, the time complexity of \textsc{InsertX} in Algorithm~\ref{alg:adaptive_hbe1} is $O(\epsilon^{-2} V(\tau) \log(1/\delta) \cdot C \cdot \log((10 k/\epsilon \tau )^d/\delta))$.
\end{lemma}


\begin{proof}


Because in \textsc{InsertX} operation in Algorithm~\ref{alg:adaptive_hbe1}, $\HBE$.\textsc{InsertX} is called for $L = O(\log((10 k/\epsilon \tau )^d/\delta))$ times, and each $\HBE$.\textsc{InsertX} takes $O(\epsilon^{-2} V(\tau) \log(1/\delta) \cdot C)$ time to complete. Therefore, the overall time complexity of  \textsc{InsertX} operation in Algorithm~\ref{alg:adaptive_hbe1} is $O(\epsilon^{-2} V(\tau) \log(1/\delta) \cdot C \cdot \log((10 k/\epsilon \tau )^d/\delta))$.
\end{proof}


\subsection{Running time of \textsc{DeleteX}}\label{sec:adaptive_multi_delete_time_app}
The goal of this section is to prove the time complexity of \textsc{DeleteX} operation.

\begin{lemma}[Restatement of Lemma~\ref{lem:adaptive_multi_delete_time}]
Given an estimator $Z$ of complexity $C$ which is $V$-bounded, the time complexity of  \textsc{DeleteX} in Algorithm~\ref{alg:adaptive_hbe1} is $O(\epsilon^{-2} V(\tau) \log(1/\delta) \cdot C \cdot \log((10 k/\epsilon \tau )^d/\delta))$.
\end{lemma}
\begin{proof}
Because in \textsc{DeleteX} operation in Algorithm~\ref{alg:adaptive_hbe1}, $\HBE$.\textsc{DeleteX} operation is called for $L = O(\log((10 k/\epsilon \tau )^d/\delta))$ times, and each $\HBE$.\textsc{DeleteX} operation takes $O(\epsilon^{-2} V(\tau) \log(1/\delta) \cdot C)$ time to complete. Therefore, the overall time complexity of  \textsc{DeleteX} operation operation in Algorithm~\ref{alg:adaptive_hbe1} is $O(\epsilon^{-2} V(\tau) \log(1/\delta) \cdot C \cdot \log((10 k/\epsilon \tau )^d/\delta))$.
\end{proof}
